Byzantine-Robust Federated Learning with Optimal Statistical Rates and Privacy Guarantees

We propose Byzantine-robust federated learning protocols with nearly optimal statistical rates. In contrast to prior work, our proposed protocols improve the dimension dependence and achieve a tight statistical rate in terms of all the parameters for strongly convex losses. We benchmark against competing protocols and show the empirical superiority of the proposed protocols. Finally, we remark that our protocols with bucketing can be naturally combined with privacy-guaranteeing procedures to introduce security against a semi-honest server. The code for evaluation is provided in https://github.com/wanglun1996/secure-robust-federated-learning.

==> app_attack.tex <==
\section{Details of Attacks}
\label{sec:append-eval-attack}

\noindent \textbf{Attacks.}~The first and second attacks are the model poisoning
attacks~\cite{fang2019local}.
%
Model poisoning attacks aim to raise the error rate of the converged model even
facing Byzantine-robust protocols.
%
In these attacks, malicious clients search for poisoning updates by solving
optimization problems.
%
We employ two of their proposed attacks targeting Krum and Trimmed Mean.
%
These two attacks are referred to as Krum Attack (KA) and Trimmed Mean Attack (TMA).
% We used their attacks designed for Krum~(\cite{blanchard2017machine}) and trimmed mean henceforth referred to as Krum Attack (KA) and Trimmed Mean Attack (TMA) separately.

The third attack we consider is a backdoor attack from~\cite{bhagoji2019analyzing}. The attack aims to inject a backdoor functionality while preserving high accuracy on the validation set.
%
Similarly, the search for the attack gradient is formalized as an optimization
problem, and the authors modify the objective function using stealth metrics to
make the attack gradient hard to detect.
%
We refer to this attack as Model Poisoning Attack (MPA).

The fourth attack is also a backdoor attack proposed
by~\cite{bagdasaryan2020backdoor}.
%
In this attack, the adversary locally trains a model using a backdoor and then
attempts to replace the global model with the local model by uploading the
difference between the target and global models.
%
We refer to the attack as Model Replacement Attack (MRA).

The fifth attack is a distributed backdoor attack (DBA)~\cite{xie2019dba},
in which the attacker manipulates updates of several clients to insert a backdoor into the global model collaboratively.

% \noindent \textbf{Clarification on Targeted Attacks for \agg.} Attentive readers might notice that the first and second attacks are designed specifically for Krum and TrimmedMean, and wonder whether it is possible to construct an attack particularly for \agg.
% %
% We argue that designing such an attack using the same idea
% from~\cite{fang2019local} is not possible, as the optimization problem becomes intractable when \agg is plugged in.
% %
% Due to the theoretically stronger robustness, we assume that it is very challenging to design targeted attacks for \agg like Krum or Trimmed Mean.
% %
% We leave it as an important future direction to design such an attack or rigorously prove its impossibility.

==> app_rt.tex <==
\section{Running Time}

\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c}
    Aggregator & Running Time (s) \\
    Average & 0.145\\ % 0.1449882984161377
    Krum & 23.748 \\ % 23.74781847000122
    Trimmed Mean & 1.219\\ %1.2188889980316162
    \textsc{Filterl2} & 1397.357\\ %1397.357472896576
    \textsc{No-Regret} & 642.246\\ %642.2461814880371
    \textsc{Bucketing Filterl2} & 1407.997\\ %1407.9973721504211
    \textsc{Bucketing No-Regret} & 2706.512\\    %2706.511966228485
    \end{tabular}
    \caption{Running time of different robust aggregators under TMA attack.}
    \label{tab:my_label}
\end{table}

==> app_xie_attack.tex <==
\section{Additional Attacks}

In this section, we evaluate the proposed robust aggregators under the attack by \citet{xie2020fall}. One can see that the new attack model does not affect the model accuracy largely for the proposed algorithms. 
% We will supply additional results for other algorithms and the new attack model~\cite{baruch2019little} in the camera ready version.

\begin{figure}[hb]
    \centering
    \resizebox{0.3\textwidth}{!}{\input{figs/main/MNIST/xie}}
    \caption{Evaluation under the attack by~\citet{xie2020fall}. The legend follows the same as in Figure~\ref{fig:main_evaluation}.}
    \label{fig:xie}
\end{figure}

==> figs/gan/legend.tex <==
\newenvironment{customlegend}[1][]{%
    \begingroup
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\begin{tikzpicture}
\begin{customlegend}[legend columns=1,legend style={align=left,draw=none, font=\footnotesize},legend entries={\textsc{GAN},\textsc{Filtering}, \textsc{No-Regret},\textsc{Bucketing-Filtering}, \textsc{Bucketing-No-Regret},\textsc{Average}, \textsc{Krum},\textsc{Trimmed Mean},\textsc{Median}}]
        \addlegendimage{mark=none,purple,line width=1pt}
        \addlegendimage{mark=none,cyan,line width=1pt}
        \addlegendimage{mark=none,green,line width=1pt}
        \addlegendimage{mark=none,black,line width=1pt}
        \addlegendimage{mark=none,gray,line width=1pt}
        \addlegendimage{mark=none,dashed,red,line width=1pt}
        \addlegendimage{mark=none,dashed,blue,line width=1pt}
        \addlegendimage{mark=none,dashed,brown,line width=1pt}
        % \addlegendimage{mark=none,dashed,darkgreen,line width=1pt}
        % \addlegendimage{mark=none,dashed,orange,line width=1pt}
        \addlegendimage{mark=none,dashed,magenta,line width=1pt}
        % \addlegendimage{mark=none,dashed,violet,line width=1pt}
\end{customlegend}
\end{tikzpicture}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> preliminary.tex <==
\section{Preliminaries: Robust Mean Estimation \& Secure Aggregation}
\label{sec:prelim}
%
In this section, we review the two main building blocks: robust mean estimation and secure aggregation in \system.

\lun{iterate over this}
\subsection{Robust Mean Estimation.} 
%
The core step in federated learning is to aggregate the individual updates from the clients.
%
The most commonly used aggregation is to average all the updates.
%
Given the threat model that some clients might be malicious, we want to estimate the mean value as close as to the true mean value without the malicious updates. 
%
There are a spectrum of works focusing on addressing the problem in the such as Krum~\cite{blanchard2017machine} and Bulyan~\cite{mhamdi2018hidden}.
%
However, all the known estimators' estimation error grows proportionally with $\sqrt{d}$ where $d$ is the parameter size of the model.
%
Such error is unacceptable in federated learning since the model size is typically tens of thousands to hundreds of thousands.

Actually, the problem is well studied in statistics under the name ``robust mean estimation'' and there already exist several robust mean estimators with dimension-free estimation error~(\cite{diakonikolas2019robust,charikar2017learning,steinhardt2018robust,cheng2019high,dong2019quantum}).
%
We present a representative aggregator namely \agg here.
%


As mentioned, \agg provides dimension-free error rate formally presented as follow.
%
\begin{theorem}
Let $\mathcal{D}$ be the honest dataset and $\mathcal{D}^{*}$ be the contaminated version of $\mathcal{D}$ by inserting arbitrary samples.
%
Suppose that $|\mathcal{D}^{*}|\leq |\mathcal{D}|/(1-\epsilon)$, and further suppose that $\textsc{Mean}[\mathcal{D}]=\boldsymbol{\mu}$ and $\|\textsc{Cov}[\mathcal{D}]\|_{op}\leq\sigma^2$. %
Then given $\mathcal{D}^*$, Algorithm~\ref{alg:filterl2} outputs $\hat{\boldsymbol{\mu}}$ s.t. $\|\hat{\boldsymbol{\mu}}-\boldsymbol{\mu}\|_2=\mathcal{O}(\sigma\sqrt{\epsilon})$ using $\textsc{poly}(n,d)$ time.
%
% $\textsc{poly}(n,d)$ that outputs $q$ with $\textsc{TV}(p^{*},q)\leq \epsilon$ and $\|\textsc{Cov}_q[X]\|\leq \mathcal{O}(\sigma^2)$.
%
% In particular, $\|\mu(p^{*})-\mu(q)\|_2=\mathcal{O}(\sigma\sqrt{\epsilon})$.
\label{thm:filterl2}
\end{theorem}

\subsection{Secure Aggregation.} 
%
Secure aggregation is a cryptographic technique developed by~\cite{bonawitz2017practical} to defend against a semi-honest server in federated learning.
%
In particular, secure aggregation allows the server to access the averaged update but prevents it from seeing individual updates from clients.
%
Thus, the server cannot launch inference attacks on the individual updates.

To better demonstrate \system, we give a high-level context on how secure aggregation works.
%
As the first step, each client generates random values for all the other clients and send each value to the corresponding client.
%
After receiving all the random values from other clients, each client sums up the received values and subtracts the values generated by itself to produce a random mask.
%
It is clear that all the masks sum up to zero.
%
Then each client blind its update with the random mask and send the blinded update to the server.
%
As the last step, the server sums up all the updates.
%
Obviously, all the masks cancel out during aggregation and the server receives the plaintext sum.

==> protocol_old.tex <==
% \vspace{-0.8em}
\section{\texorpdfstring{\system}{F2ed-Learning}}
\label{sec:system}
% \vspace{-0.6em}

%In this section, we formally present our main protocol: \system.
The full protocol of \system will be given \A~\ref{alg:protocol}, and we first
summarize its high-level workflow in \F~\ref{fig:pipeline}(a): \system provides
bidirectional defense, defending against the semi-honest server through secure
aggregation (marked in \textcolor{red}{red}) and malicious clients with the
robust mean estimator \agg (marked in \textcolor{blue}{blue}).
\F~\ref{fig:pipeline}(b) formulates \agg, the details of which are presented in
\S~\ref{sec:protocol1}. We now introduce \system and formally
establish the robustness and security guarantees in \S~\ref{sec:analysis}.


% All the proofs are deferred to the Appendix ??? due to the space limitation.

\subsection{\texorpdfstring{\system}{F2ed-Learning}: Byzantine-Robust Privacy-Preserving FL}
\label{sec:protocol1}

%
The complete \system protocol is presented in Algorithm~\ref{alg:protocol}.
%
\system iteratively executes the following steps: (1) the server broadcasts the
global model to the clients; (2) the clients train the global model using their
local data; (3) clients within the same shard use a secure aggregation protocol
to upload the mean of their updates to the server; (4) the server aggregates the
received updates using robust mean estimation; and (5) the server updates the
global model with the aggregated global update.
%
We highlight steps (3) and (4) newly proposed in \system.
%
% Robust estimation and secure aggregation defend against Byzantine clients and semi-honest server separately.
% %
% However, we need both protections simultaneously in the real world.
% %
% To do so, we need to reconcile robust mean estimator and secure aggregation.
% %
% However, they are intrinsically contradictory because robust mean estimation needs to check individual updates but secure aggregation only allows the server to check the aggregated result. 
% %
% To reconcile the two building blocks, we shard the clients, execute secure aggregation within each shard and run the robust estimator on the updates from each shard.
% %
% The complete protocol is shown as below.


% \vspace{5pt}

\vspace{-1em}
\noindent \textbf{Sharded Secure Aggregation (lines 7--8, 10, 13).}~Secure
aggregation is developed by~\cite{bonawitz2017practical} to defend a
semi-honest server in FL. Secure aggregation allows the server to obtain the sum
of the clients' updates but cryptographically conceals individual updates. To
begin, each client samples random values and transmits the values to other
clients in the same shard (lines 7–8).
%
Notably, secure aggregation and cryptographic protocols demand that client
updates be integers while transmitting them via modular operation. Because each
client's model update uses float numbers, we first quantize before secure
aggregation (line 10).
%
After receiving all values from other clients, each client adds the received
values together and subtracts its own to produce a random mask (line 10). Each
client blinds its local update with the random mask and sends the blinded update
to the server (line 11). The server then aggregates all blinded updates and
obtains the plaintext of the summed update (line 13). All masks cancel
out during aggregation, and the server receives the plaintext sum. Secure
aggregation ensures client privacy by hiding each client in the aggregation of other
clients.

Note that in our threat model, vanilla secure aggregation is insufficient since
it provides no protection for the server.
%
Due to the total concealment of the individual updates, the server is unable to
identify the malicious clients even after detecting the attack.
%
To address the issue, we, therefore, propose that clients are partitioned into multiple
shards (lines 7–8) and secure aggregation be performed within each shard.
%
The size of the shards is a trade-off between server and client protection.
%
The smaller the shard size, the more information the server reveals, making it
easier to defend against Byzantine malicious clients and harder to combat the
semi-honest server.
%
The trade-off is elaborated in \S~\ref{sec:analysis}.
% \fixme{this discussion is missing.}

% The fundamental step of Byzantine-robust FL is to reliably estimate the true
% mean of the benign updates, even when some malicious clients are present.
% Averaging, the most widely used aggregator, has been shown to be vulnerable to
% even a single rogue client. However, previous research in this sector (e.g.,
% Krum~\cite{blanchard2017machine} and Bulyan~\cite{mhamdi2018hidden} suffer from a
% dimension-dependent estimation error. Notably, such dimension-dependent error
% can impose an intolerably high cost even when training a three-layer MLP on
% MNIST, let alone more complex tasks and models such as VGG16 or ResNet50.

% \vspace{-0.3em}
\smallskip
\noindent \textbf{Robust Mean Estimation (line 14).}~The fundamental step of
Byzantine-robust FL is to estimate the true mean of the benign updates as
accurately as possible, even when some malicious clients are present. Averaging,
the most widely used aggregator, has been shown to be vulnerable to even a
single malicious client. However, existing works in this field (e.g.,
Krum~\cite{blanchard2017machine} and Bulyan~\cite{mhamdi2018hidden}) suffer
from a \textit{dimension-dependent} estimation error. Note that such
dimension-dependent error can impose an intolerably high cost even when training
a three-layer MLP on MNIST, let alone more complex tasks and models such as
VGG16 or ResNet50.

% It is worth noting that robust mean estimation has been extensively investigated
% in statistics, with the goal of developing a robust mean estimator with
% dimension-free estimate error (Diakonikolas et al., 2019; Charikar et al., 2017;
% Steinhardt, 2018; Cheng et al., 2019; Dong et al., 2019). However, due to their
% strong requirement for i.i.d. data, such dimension-free mean estimators were not
% used.

% \fixme{It is worth mentioning that in statistics, robust mean estimation has been
% well-studied, with the goal of delivering a robust mean estimator with
% dimension-free estimation error~\cite{diakonikolas2019robust,
%   charikar2017learning, steinhardt2018robust, cheng2019high, dong2019quantum}.
% However, due to their strong requirement for i.i.d. data, such dimension-free mean
% estimators were not used.}

\system, in particular, incorporates a well-known robust mean estimator:
\agg~\cite{steinhardt2018robust}. We formulate \agg in
\A~\hyperref[fig:pipeline]{2}. \agg assigns each client's update a weight and iteratively
updates the weights until the weights for malicious clients' updates are sufficiently
small. \agg provides a dimension-free error rate that is formally
presented as follows.

\begin{theorem}[\cite{steinhardt2018robust}]
Let $D$ be the honest dataset and $D^{*}$ be the contaminated version of $D$ by inserting malicious samples.
%
Suppose that $|D^{*}| < |D|/(1-\epsilon)$, and further suppose that $\textsc{Mean}[D]=\boldsymbol{\mu}$ and $\|\textsc{Cov}[D]\|_{op}\leq\sigma^2$. %
Then, given $\mathcal{D}^*$, Algorithm~\hyperref[fig:pipeline]{2} outputs $\hat{\boldsymbol{\mu}}$ s.t. $\|\hat{\boldsymbol{\mu}}-\boldsymbol{\mu}\|_2=\mathcal{O}(\sigma\sqrt{\epsilon})$ using $\textsc{poly}(n,d)$ time, where $\epsilon$ is the fraction of malicious data and $\epsilon < \frac{1}{2}$.
%
% $\textsc{poly}(n,d)$ that outputs $q$ with $\textsc{TV}(p^{*},q)\leq \epsilon$ and $\|\textsc{Cov}_q[X]\|\leq \mathcal{O}(\sigma^2)$.
%
% In particular, $\|\mu(p^{*})-\mu(q)\|_2=\mathcal{O}(\sigma\sqrt{\epsilon})$.
\label{thm:filterl2}
\end{theorem}


% \vspace{-0.4em}
Although Algorithm~\hyperref[fig:pipeline]{2} runs in polynomial time, the
per-round time complexity is $\mathcal{O}(nd^2)$ if implemented with power
iteration.
%
Given $d$ is large, the running time is still quite expensive in practice.
%
To address the problem, we divide the update vectors into $k$ sections and apply
the robust estimator to each section.
%
The acceleration scheme reduces the per-round running time to
$\mathcal{O}(nd^2/k)$, but increases the estimation error to
$\mathcal{O}(\sigma\sqrt{\epsilon k})$.
%
For instance, if we take $k=\sqrt{d}$, the per-round running time becomes
$\mathcal{O}(nd\sqrt{d})$, while the estimation error increases to
$\mathcal{O}(\sigma\sqrt[4]{\epsilon^2 d})$.
%
Despite the tradeoff for acceleration, \agg maintains the known optimal
estimation error and outperforms other robust FL protocols by several orders of
magnitude, as shown in \S~\ref{sec:evaluation}.



\subsection{Robustness \& Security Analysis}
\label{sec:analysis}

In this section, we rigorously prove the security and robustness guarantee of \system.


% \vspace{-0.3em}
\smallskip
\noindent \textbf{Security Guarantee.}~We first give the security guarantee of
\system as follows. Intuitively, the centralized server learns nothing more
about the clients than the averaged updates from the shards. Thus, each client's
update is hidden by the rest clients in its shard.
%
% The proof is deferred to~\ref{sec:cor1}.
%
\begin{corollary}[Security against semi-honest server]
%
Let $\Pi$ be an instantiation of \system, there exists a PPT (probabilistic polynomial Turing machine) simulator $\textsc{Sim}$ which can only see the averaged updates from the shards. For all clients $\mathcal{C}$, the output of $\textsc{Sim}$ is computationally indistinguishable from the view of that real server $\Pi_\mathcal{C}$ in that execution, i.e., $\Pi_\mathcal{C} \approx \textsc{Sim}(\{ \textbf{g}_t^{H_j} \}_{j \in [p]})$.

\label{cor:sec}

\end{corollary}

We present the proof for Corollary~\ref{cor:sec} in Appendix~\ref{sec:proof-corollary1}.
% \input{proof-corollary1}

% \vspace{-5pt}
% \begin{proof}
% %
% \fixme{Put it to appendix.}
% The transcript of the server is the updates from the sharded clients.
% %
% Hence, Corollary~\ref{cor:sec} is equivalent to the following lemma since the PPT can split the aggregated updates into several random shares which is computationally indistinguishable from the true transcript. The detailed proof of the lemma can be found in Appendix~\ref{sec:proof-lemma1}.

% \begin{lemma}[Lemma 6.1 in~\cite{bonawitz2017practical}]
% Given the number of the shards $p$, the parameter size $d$, the group size $q$, and the updates $\textbf{g}^{H_i}$ where $\forall i\in[p], \textbf{g}^{H_i}\in \mathbb{Z}^d_q$, we have 
% \begin{equation*}
% \begin{split}
%     &\{\{\textbf{u}_{ij}\overset{\$}{\leftarrow}\mathbb{Z}_q^d\}_{i<j}, \textbf{u}_{ij}\coloneqq -\textbf{u}_{ji} \; \forall i>j \quad : \{\textbf{g}^{H_i}+\sum_{j\in[p]\slash i}\textbf{u}_{ij} \pmod{q}\}_{i\in[p]}\}
%     \\ \equiv &\{\{\textbf{v}_i\overset{\$}{\leftarrow}\mathbb{Z}_q^d\}_{i\in[p]}~s.t.~ \sum_{i\in[p]}\textbf{v}_i=\sum_{i\in[p]}\textbf{g}^{H_i} \pmod{q} \quad : \{\textbf{v}_{i}\}_{i\in[q]}\}
% \end{split}
% \end{equation*}
% where "$\equiv$" denotes that the distributions are identical.
% \label{lem:sec}
% \end{lemma}



% % \noindent\textbf{Base case:} When $n=2$, the first elements of two distributions are both uniformly random.
% % %
% % The second element is the sum minus of the corresponding first element.
% % %
% % Thus the distributions are identical.

% % \noindent\textbf{Inductive Hypothesis:}
% % When $n=k$, the lemma holds.

% % \noindent\textbf{Inductive Step:}
% % % If we ignore all the randomness from and for client $k+1$, 
% % According to the inductive hypothesis, the left and right distributions of the first $k$ clients are indistinguishable.
% % %
% % We follow the protocol to generate the left transcript when the $(k+1)^{th}$ client is added to the shard.
% % %
% % To deal with the right-hand-side transcript, we first add the same randomness as left-hand-side to the first $k$ updates and then subtract them from the total sum to get the $(k+1)^{th}$ update.
% % %
% % It is easy to prove that the first $k$ updates on the left and right follow the same uniformly random distribution and the $(k+1)^{th}$ update is the difference between the total sum and the sum of the first $k$ updates.
% % %
% % Hence, the left and right transcripts are indistinguishable.
% % To add the $(k+1)^{th}$ client to the left-hand-side distribution, we follow the protocol to add randomness to the first $k$ clients.
% %
% % To keep the indistinguishability, we add the same randomness to the right-hand-side distribution. 
% % %
% % For the left-hand-side, we follow the protocol to generate the $(k+1)^{th}$ update while for the right-hand-side, we subtract the first $k$ updates from the total sum to generate the $k^{th}$ update.
% % %
% % It is easy to prove that the left-hand-side distribution 
% % For the right-hand-side distribution, we subtract 
% % Hence, after adding two independently uniformly random values, the distributions are still identical.
% % %
% % The value for the $k+1^{th}$ client is the sum minus $k$ uniformly random values.
% % %
% % Thus, the two distributions are still identical.

% \end{proof}

% \vspace{5pt}

% \vspace{-0.3em}
\smallskip
\noindent \textbf{Robustness Guarantee.}~We now give the formal robustness
guarantee of \system. The proof involves a trivial application of
Theorem~\ref{thm:filterl2} so we omit it here.
% Intuitively, if the number of shards containing malicious clients is small enough, \system can provide mean estimation with dimension-free error (or quad-root error with the acceleration).
%
% The proof is deferred to Appendix~\ref{sec:cor2}.
%

\begin{corollary}[Robustness against Byzantine adversaries]
Given the number of clients $n$, the number of shards $p$, and the fraction of corrupted clients $\eta$, \system provides a mean estimation with dimension-free error as long as $\eta n < \epsilon p$, where $\epsilon < \frac{1}{2}$ is the tolerance of FilterL2 given in Theorem~\ref{thm:filterl2}.
\label{cor:robust}
\end{corollary}

We present the proof for Corollary~\ref{cor:robust} in Appendix~\ref{sec:proof-corollary2}.
% \input{proof-corollary2}

% \begin{proof}
% In the following analysis, we assume that the updates from the shards follow an IID distribution.
% %
% The reasonableness of the assumption is further discussed in Section~\ref{sec:iid}.

% The fraction of malicious shards is bounded by the worst case where each malicious client is exclusively assigned to different shards: $\epsilon'\leq \frac{\epsilon n}{p}\leq \frac{1}{12}$.
% %
% Given the assumption above, we have satisfied all the requirements in Theorem~\ref{thm:filterl2}.
% %
% Hence, \system provides a mean estimation with dimension-free error as long as $12\epsilon n < p$.

% \end{proof}

% \vspace{-5pt}

% \vspace{-0.5em}
\smallskip
\noindent \textbf{Remark.}~Given the formal security and robustness guarantees,
it is clear that \system enables easy calibration of the server's or clients'
protection.
%
\system, in particular, can tolerate up to $\lfloor{\epsilon p} \rfloor$
malicious clients and conceal each honest client's update in the mean of
$\lfloor\frac{n}{p}\rfloor$ updates.
We present further discussion on the shard size $p$ in Appendix~\ref{sec:shard-size-append}.
%\fixme{To address the challenge of
%  incompatibility between robust estimator and secure aggregation, \system uses
%  sharding to achieve a good balance between robustness and security levels.}
As illustrated in \F~\ref{fig:pipeline}, \system employs a novel
sharding scheme to overcome the incompatibility between a robust estimator and
secure aggregation. 
% The value of $p$, denoting the number of shards,
% primarily affects the robustness and security provided by \system.
% % 
% If the number of benign shards is less than the number of
% malicious shards (i.e., $p \leq 2 \eta n$), FilterL2's
% requirement on the fraction of malicious shards $\epsilon < \frac{1}{2}$ may
% not hold. That is, \system may not exclude malicious shards if $p$ is
% insufficiently large. However, if $p$ is too large, implying that the
% number of clients in each shard is small, the semi-honest server is more likely to 
% infer the clients' private updates from the aggregations of
% the shards. In practice, $p$ should be determined by the total
% number of clients, the desired level of security and robustness, and
% the nature of the FL task. See evaluation in \F~\ref{fig:f6} for various numbers of shards.

% Attentive readers might notice that the robustness tolerance is lower than when there is no sharding.
% %
% We argue that it is an almost unavoidable cost because if we can have the same robustness tolerance as the no-sharding case, then we can design a robust estimator for partially aggregated samples with the same tolerance.
% %
% As the latter problem is unsolved, we deem it extremely challenging to further increase the tolerance in our scenario.

